Privacy Engineering Meets Software Engineering. On the Challenges of Engineering Privacy ByDesign

Current day software development relies heavily on the use of service architectures and on agile iterative development methods to design, implement, and deploy systems. These practices result in systems made up of multiple services that introduce new data flows and evolving designs that escape the control of a single designer. Academic privacy engineering literature typically abstracts away such conditions of software production in order to achieve generalizable results. Yet, through a systematic study of the literature, we show that proposed solutions inevitably make assumptions about software architectures, development methods and scope of designer control that are misaligned with current practices. These misalignments are likely to pose an obstacle to operationalizing privacy engineering solutions in the wild. Specifically, we identify important limitations in the approaches that researchers take to design and evaluate privacy enhancing technologies which ripple to proposals for privacy engineering methodologies. Based on our analysis, we delineate research and actions needed to re-align research with practice, changes that serve a precondition for the operationalization of academic privacy results in common software engineering practices.

==> appendices/AgileMethodsHistory.tex <==
\subsection{Agile development: A New World}
Since the beginning of software engineering in the late 60s, a variety of management and engineering literature proposed wildly different models on how to produce software. Until the 1990s, structured processes, such as the waterfall or spiral model, dominated the industry. These models rely on rigorously regimented practices, extensive documentation, and detailed planning and management \cite{EstlerNFMS14}. In \emph{waterfall models}, as the US Department of Defense standardized the term, software projects have a clear beginning during which the requirements and design are settled, and a final stage during which a version of a software is tested and released to its users. 

Starting with the 1980s, and continuing with the 1990s, programmers started proposing more \emph{lightweight} models that promoted greater autonomy for developer teams, questioning the predominantly managerial approaches to software development. Scrum, Rational Unified Process, Extreme Programming presented turning points in these developments. Some of these methodologies focus on techniques (e.g., pair-programming), while others focus on managerial processes (e.g., stakeholder involvement, stand-up meetings), with an overall emphasis on continuous testing (starting with test codes and extending to integration testing), communication and visibility of progress (Parson 2011). 

We use \emph{agile methodologies} as an umbrella term to refer to this latter variety of approaches to software development that contrast with what are called Big Design Up Front models, and that emphasize iterative customer centered engineering of functionality. We shorthand these methods as agile inspired by one of these proposals which culminated in what was titled the ``Manifesto for Agile Software Development'' in 2001 \cite{beckBCCFGHHJKMMMSST2001}. The supporters of this manifesto value:
\begin{quote}
Individuals and interactions over processes and tools\\
                               Working software over comprehensive documentation\\
      Customer collaboration over contract negotiation\\
    	        Responding to change over following a plan \cite{beckBCCFGHHJKMMMSST2001}.\\

\end{quote}

Like many of its contemporaries, the manifesto underlines a ``no design up front'' attitude. Instead, it proposes to produce software in much shorter iterations (weeks vs years, or multiple times a day), in greater simplicity (always do the simplest thing that could possibly work and don't design more than what you need right now), and continuous code reviews \cite{FoxP13}. This leads to increased emphasis on modularity, incremental design, iterations in feature development that are open to changing requirements, and continuous deployment, i.e., releasing code as frequently as possible. Another important effect is the removal of documentation efforts, assuming that development must modularize and simplify code, ideally, to the extent of making documentation redundant. 

Agile methods are as much about development efficiency as they are about the success of software based businesses. In addition to enabling customer centricity, agile methods promise to give companies control over the costs of maintenance, monitoring, and support. Instead of waiting for the release of new versions, users can benefit from continuous updates. This produces a big advantage in an industry where as much as 60 percent of software costs are for maintenance, and of those costs 60 percent are for adding new functionality to legacy software (Armando and Patterson 2013).

Some methods make the connection between business interests and development methodologies even more evident. Especially development methods inspired by processes used in traditional manufacturing, e.g., Kanban, lean manufacturing were key to aligning business models, key performance indicators (KPIs) with rapid feature development driven by feedback from users or customers. As a result, data that could be used to measure user interactions and interest became a necessary part of optimizing features, fulfilling KPIs and pivoting companies effectively towards more promising business models.

Finally, despite their anti-managerial gist, proposals for agile methodologies were aligned with then new management theories which erred on the side of ``multidisciplinary teams''  that work more like a rugby team engaged in iterative experimentation across all phases of production simultaneously as a way to achieve speed and flexibility in production. In addition to enabling programming and business on demand, these methods were invaluable in addressing the inflexibility of planned development that proved to lead to grand failures and brittleness in managing uncertainty. Agile methodologies also promoted a much more experimental approach to software engineering, relying on user data and feedback for enabling these experiments.


==> appendices/EPbDMethodologies.tex <==




\subsection{PbD as practice: Privacy papers and the SDL / (micro)services}


\subsubsection{Risk assessment/Threat modeling}



The LINDDUN methodology is an approach for modeling privacy threats \cite{DengWSPJ11}. The methodology includes the anti-property or threat for two types of privacy properties: soft (content unawareness, policy and consent noncompliance) and hard (likability, identifiability, non-repudiation, detectability, and disclosure of information). LINDDUN is influenced by STRIDE \cite{Shostack14}, a security modeling method with trees of threats and data flow diagrams created for each category of threats. It is possible to use the LINDDUN as a reference guide for privacy threats but lacks the mapping to a software development process and a comprehensive view of the organizational goals linked with the privacy goals.

\subsubsection{Goal-oriented} 



In their work, Liu and colleagues present privacy and security from the point of view of requirements engineering \cite{LiuYM03}. Privacy is a non-functional requirement that affects the design of the system, which is modeled with i*, a goal-oriented modeling method. Their approach is to transform OECD's categories into goals and to then, create a reference catalogue with privacy solutions addressing each privacy goal. The catalogue is high-level motivational analysis (consisting of actors who have goals and soft goals, and who take actions to achieve their goals). The actions for satisfying the different goals are not universal and are arbitrarily chosen to show a proof-of-concept for modeling privacy requirements. The works merits include contextual analysis capabilities and structural consistency based on a requirements engineering modeling method. With the modeling method, it is possible to present dependencies between goals (of the same actor or of different actors), to model the viewpoints of different actors and other non-functional requirements.


PriS proposes a holistic approach that connects `high-level' organizational goals and `privacy-compliant' IT systems \cite{KalloniatisKG2008}. PriS first models privacy requirements from an organizational point of view in the form of organizational goals (GORE) and then, using seven predefined privacy-process patterns describes the impact of the privacy goals on the organizational processes and the IT systems. The Formal PriS method also defines four activities to carry out the design: (1) elicit privacy-related goals, (2) analyse the impact of privacy goals on organizational processes, (3) model affected processes using privacy-process patterns, (4) identify the techniques that best support/implement privacy-related processes. The authors identify the gap between design and implementation and the lack of support given to developers to implement privacy requirements into their systems. PriS is a methodology rather than a recipe book -- it uses models and principles of refinement and abstraction between levels to connect different areas/domain involved in system design. However, PriS lacks the mechanism to integrate this design process into an iterative software development. PriS does not consider the type of software system to be developed: there is no discrimination between a monolith and a service-oriented system, hence, there are no guidelines how to reason about modular ever-changing system. Also, even though, the authors list several PETs ``implementing'' the eight privacy requirements, the list is limited to technologies and not to classes of technologies, which makes it unsuitable for extending. The leap between the privacy process patterns and the PETs is non-trivial and even though the authors set for themselves the goal to provide a methodology that does not give a static recipe but a heuristics-based holistic approach to integrate privacy into IT systems, it is unclear how to break out of the pre-defined privacy requirements, the pre-defined privacy-process patterns, or the pre-defined PETs mapping. Privacy is loosely defined: it is a specialized organizational goal or a requirement. However, there are eight privacy goals that are assumed to be a given even though the first activity in the methodology is to identify privacy goals (authorization, authentication, identification, anonymity, data protection, pseudonymity, unlinkability, and unobservability).

Hansen et al. introduced the notion of protection goals to create ``a feature-complete model for evaluating an IT system's impact on all aspects of privacy and data protection'' \cite{HansenJR15}. The privacy goals are six and include three well-established goals from security (confidentiality, integrity, availability, or CIA) and the newly relevant goals of privacy and data protection (unlikability, transparency, and intervenability). The authors discriminate between privacy and data protection; privacy take on the perspective of an individual, whereas data protection is an organization-centered view.  The goals are complimentary w.r.t. achieving privacy in an ideal world but as the authors point out, these goals are contradictory and depending on the technology that implements them, might be exclusive. For example, transparency and linkability are of conflicting nature, as the former requires monitoring of the actual processing by, for example, logging various actions, but the latter promotes avoidance of such information being recorded to minimize the risk of misuse. The work mentions the challenges of using external services by providing data in the clear only to introduce some techniques (e.g. secure computation and homomorphic encryption). The challenges for software developers to reason about privacy and data protection are not mentioned.


\subsection{Software Development/System Design}

Hoepman defines privacy design strategies to help IT engineers solve recurring software development problems in the light of 'privacy-by-design' development \cite{Hoepman14}. The first observation we make is that the author assumes that privacy and data protection are synonyms. From then on, to aid the IT architects, Hoepman derives privacy design from legislation (e.g., OECD guidelines, the 1995 European data protection directive) and maps them to (privacy) design patterns that help implement the strategy. There are eight privacy design strategies related either to the data (minimize, separate, aggregate, hide) or to the process (inform, control, demonstrate, enforce). Our next observation is that the privacy design patterns are not complete; there are some suggestions (select before collect, mix networks, etc.) but the author gives no comprehensive list later to be categorized as a pattern for one or another strategy. Moreover, the privacy design patterns are not software design patterns. For example, encryption (a privacy pattern for the hide strategy) is a technique rather than ``a schema for refining the subsystems or the components of a software system, or the relationship between them'', which is the definition of a design pattern the author adopted in their paper. For a non-expert privacy engineer, this terminology would be misleading. Other privacy strategies lack design patterns altogether, e.g. separate. Moreover, the strategies do not describe how to engineer privacy by design in an agile software development process or how to compose applications from various components. There is no mention of how to evolve a software iteratively, which is the pre-dominant industry case.


Spiekermann and Cranor discuss the practical implications of engineering privacy and what the shift from privacy from the physical to the digital world might entail \cite{SpiekermannC09}. In their work, the authors propose the use of a privacy sphere - a privacy space for users, recipients, and a joint sphere. The spheres help us reason about the privacy constraints and concerns within the boundaries of each sphere. Moreover, Spiekermann and Cranor devise a system design method for including privacy in the design. At the first two stages of the system design, the authors propose that privacy be addressed with the help of policies. At the last two stages - with the help of architectural choices. The policies are a light-weight privacy mechanism as they ensure not so much privacy as compliance. As for the architectural choices, they are explained in detail but are disconnected from the practical work of a developer, i.e. who would find them as a prescription only to a subset of architectural choices they need to make, hence, rendering the architectural choices unactionable. A curious caveat in this work is the term privacy-friendly systems, that the authors coined to name systems that include privacy in their design but not necessarily in the traditional privacy-preserving or enhancing meaning that is mostly in use today.

Al-Momani et al. present a software development process (V-model) augmented for engineering privacy \cite{Al-MomaniKSKB19}. The privacy-aware V-model, called W-model, starts with privacy impact assessment in order to elicit privacy threats and to find countermeasures to remedy these threats. The W-model introduces two privacy-centric stages: privacy analysis and privacy-enhanced architecture. All the other stages of the classic V-model are ``privacy-enhanced.'' The privacy analysis during the W-process is when the privacy engineers elicit the privacy threats and select countermeasures for them. The countermeasures should be integrable in the system and compatible with other countermeasures, which are requirements not often mentioned regarding PETs when methodologies on PbD explain how to select the right one for the job. The next step, privacy-enhanced architecture, is dedicated to design a high-level and a low-level system architecture that meets the business and privacy requirements. However, the design phase and the implementation phase are disconnected and even though there is short mention on how privacy and systems engineers resolve issues arising during the implementation phase, the recommendation is that the interaction between system and privacy engineers should be on critical aspects in order to increase the time-efficiency. The claim of the authors is that the enhanced privacy culture of the companies via the component "environment and infrastructure" will reduce unnecessary communication. The paper mentions nothing regarding services and modules that interact with the PETs, only that the PETs need to be integrable in a system.


PEARs attempts to answer the question how to engineer PbD on the architectural level of an application \cite{Kung14}. As most software architecture text, it's abstract and completely out of the blue, no idea where the architectural tactics and patterns come from. Kung proposes to use a separation between NFR (how the system does it) and FR (what the system does) which is arbitrary (because such a separation does not exist). For example, FRs includes purpose limitation. Why? Why this is not an NFR? NFRs include minimization. Why? Then, the architecture is supposed to be related to some tactics that are associated with technologies and patterns. There are 4 tactics mentioned in the paper - minimization, enforcement, accountability, modifiability (unjustified where they come from). My guess is that the NFR are the source for the tactics, but this is not written explicitly. It's written that the architecture depends of NFRs but the 4 tactics are just examples and not an exhaustive taxonomy of other NFRs that can be translated into tactics for the architecture, even though the Kung describes these tactics as a proposal. The selection of the right tactics is said to be "art of selecting " and to depend of the available PETs and the cost effectiveness. No further intuition is given how to select. The paper includes 3 examples of patterns (user data confinement, hippocratic management, isolation) that are unrelated to the 4 tactics. Architecture is supposed to be evaluated with a PIA; there are 5 sentences in total that describe how this evaluation will be done. The PbD process that integrates architectural design is a linear except for one loop that connects the architecture and the privacy FRs. There is no development in the PbD process, neither the process is considered to be of any iterative nature. The process ends with the evaluation of privacy (PIA). There is no mention of composition of the software (services), how to integrate changes, context of use, development activities.





==> appendices/EPbDTable.tex <==
\begin{table*}[t]
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|}
        \hline
        
        \textbf{} & \rotatebox{90}{\textbf{Services}} & \rotatebox{90}{\textbf{Waterfall}} &  \rotatebox{90}{\textbf{Integration}} & \rotatebox{90}{\textbf{Changes}}  & \rotatebox{90}{\textbf{Heuristics}} & \rotatebox{90}{\textbf{Prescribe}}  & \rotatebox{90}{\textbf{\makecell{Minimize\\data}}} & \rotatebox{90}{\textbf{\makecell{Mapping\\to PETs}}}  & \rotatebox{90}{\textbf{\makecell{Risks/\\threats} }}& \rotatebox{90}{\textbf{\makecell{Goal-\\oriented} }} & \rotatebox{90}{\textbf{\makecell{Context \\of use}} } & \rotatebox{90}{\textbf{\makecell{Intended \\audience}} }\\ \hline
        
        \multicolumn{13}{|c|}{\textbf{Academic publications}}  \\ \hline 
        
        Hoepman (Privacy strategies) \cite{Hoepman14} & \Circle & \RIGHTcircle & \Circle & \Circle & \CIRCLE & \RIGHTcircle  & \RIGHTcircle & \CIRCLE  & \Circle  & \Circle & \Circle & Eng \\ \hline
        
        Deng et al. (LINDDUN) \cite{DengWSPJ11} & \Circle &  \CIRCLE & \Circle  &  \Circle &  \Circle &  \CIRCLE & \Circle & \CIRCLE & \CIRCLE &  \Circle & \Circle & Org/Academic \\ \hline
        
        Spiekermann and Cranor \cite{SpiekermannC09} & \CIRCLE & \CIRCLE &  \Circle &  \Circle &  \Circle &  \CIRCLE & \Circle & \Circle & \Circle & \Circle & \RIGHTcircle & Eng/Academic\\ \hline
                
        PRIAM \cite{DeM16} & \CIRCLE & \CIRCLE &  \Circle &  \Circle &  \Circle &  \CIRCLE & \RIGHTcircle & \Circle & \CIRCLE & \Circle & \CIRCLE & Org \\ \hline
                
        Hansen et al. (Protection goals) \cite{HansenJR15}  &  \CIRCLE & \CIRCLE &  \Circle &  \Circle &  \Circle &  \CIRCLE & \RIGHTcircle & \Circle & \Circle & \RIGHTcircle & \Circle & Org/Academic\\ \hline
        
        G\"urses et al. (EPbD) \cite{GursesTD11,GursesTD15} &  \Circle &  \CIRCLE &  \Circle & \Circle &  \CIRCLE  & \Circle  &  \CIRCLE  &\CIRCLE & \CIRCLE  &  \Circle &  \Circle & Org/Eng\\ \hline
        
        Al-Momani (W process) \cite{Al-MomaniKSKB19} & \Circle & \CIRCLE &  \Circle &  \RIGHTcircle &  \RIGHTcircle &  \Circle & \RIGHTcircle & \Circle &  \Circle & \CIRCLE & \Circle & Eng/Org/Academic \\ \hline
        
        Bernsmed (Applying EPbD)\cite{Bernsmed16}  & \CIRCLE & \CIRCLE & \Circle  &  \CIRCLE  &  \Circle &  \CIRCLE & \Circle & \Circle & \Circle & \Circle & \CIRCLE & Org \\ \hline
        
        Liu et al. (i*) \cite{LiuYM03} & \Circle & \CIRCLE &  \Circle &  \Circle &  \Circle &  \Circle & \Circle & \Circle &  \Circle & \CIRCLE & \CIRCLE & Org/Academic \\ \hline
        
        Kalloniatis (PriS method) \cite{KalloniatisKG2008} &  \Circle & \CIRCLE &  \Circle &  \RIGHTcircle &  \RIGHTcircle &  \Circle & \RIGHTcircle & \Circle &  \Circle & \CIRCLE & \Circle & Eng/Org/Academic \\ \hline
        
        
        Kroener and Wright \cite{KroenerW14} & \multicolumn{12}{|c|}{SoK\footnote{SoK - Summarization of Knowledge. We use the term in the broad sense to mean that the work provides an overview of the field.}  focused on the area of privacy by design in general} \\ \hline 
        
        Wueyts et al. \cite{WuytsSLJ19} & \multicolumn{12}{|c|}{SoK focused on threat elicitation} \\ \hline \hline
        
        
        \multicolumn{13}{|c|}{\textbf{Standards}}  \\ \hline 
        
        ISO 27550 \cite{ISO27550}  & \CIRCLE & \CIRCLE & \CIRCLE  &  \CIRCLE  &  \RIGHTcircle &  \Circle & \CIRCLE & \RIGHTcircle & \RIGHTcircle & \CIRCLE & \RIGHTcircle & Org/Eng \\ \hline
        
        OASIS PMRM \cite{PMRM13} & \CIRCLE  & \RIGHTcircle & \RIGHTcircle  &  \CIRCLE  &  \Circle &  \CIRCLE & \CIRCLE & \Circle & \RIGHTcircle & \Circle & \CIRCLE & Org/Eng \\ \hline
        
        Risk assessment in federal systems \cite{NISTIR8062} & \Circle & \Circle & \Circle  &  \Circle  &  \Circle &  \RIGHTcircle & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & Legal \\ \hline
        
        OASIS Cavoukian \cite{CavoukianCJSDFFF14}  & \CIRCLE & \RIGHTcircle & \Circle  &  \Circle  &  \Circle &  \CIRCLE & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & Org \\ \hline
        
        PRIPARE \cite{NotarioCMAMAKKW15}  & \Circle & \Circle & \Circle  &  \Circle  &  \Circle &  \CIRCLE & \Circle & \Circle & \CIRCLE & \CIRCLE & \CIRCLE & Org \\ \hline
        
        NISTIR 8062 \cite{NISTIR8062}  & \Circle & \Circle & \Circle  &  \Circle  &  \Circle &  \RIGHTcircle & \Circle & \Circle & \CIRCLE & \Circle & \CIRCLE & Org/Legal \\ \hline
    
    \end{tabular}
    
    \caption{Analysis of different engineering privacy by design methodologies according to twelve criteria. We used the following encoding: \Circle - the work does not consider or present this dimension, \RIGHTcircle - the work mentions this dimension but does not center around it, \CIRCLE - the work revolves around and analyzes in detail this dimension.}
    \label{table: epbd-methodologies-all}
    
\end{table*}


==> appendices/Services.tex <==
% !TeX root = ../Agile_PbD.tex
A service is an overloaded term in the literature. 
We present here the definitions from the service science and the service-oriented computing communities. 

The service-oriented computing paradigm defines services as ``self-describing, platform-agnostic computational elements that support rapid, low-cost composition of distributed applications'' \cite{Papazoglou03}.
Service-oriented computing has been extended recently to microservices.
A microservice is still a service but highly specialized and independent \cite{DragoniGLMMMS17}
The definition of microservices vary but stay within the bounds of ``independent deployment and isolated development'' \cite{microservices}.
The most recent research in the area  push the boundaries on how small a (micro)service can be. 
These inquiries include the concept of serverless computing, sometimes called a function-as-a-service, \cite{BaldiniCCCFIMMRSS17} and questions on how small a computation outsourced to a cloud can be if it still needs to make sense \cite{LeeO19}.

Microservices architecture is a software architecture in which components are lightweight microservices that communicate through heterogeneous protocols \cite{DragoniGLMMMS17}.
The composition of microservices requires coordination done via an orchestration or a choreography composition pattern \cite{DragoniGLMMMS17}. 
In the case of orchestration, there is an engine that orchestrates the microservices and leaves less logic in the individual computing units who to contact next.
In the case of choreography, the individual microservices have the embedded logic that they use to invoke other microservices \cite{CernyDT17}. 
According to Alshuqayran et al. some of the pros of the microservices architecture are increase in agility, developer productivity, resilience, scalability, reliability, maintainability, separation of concerns, and ease of deployment \cite{AlshuqayranAE16}. 
There are, however, challenges to the microservices architecture, i.e., service discovery, security management, communication optimization, data sharing, and performance .

Moreover, the \textit{context} of the system, i.e. how the microservices are used in a full system, disappears when a monolith is broken into the smallest pieces that still hold together \cite{CernyDT17}.
Each individual microservices maintain only its own context, meaning, it has a consistent state within itself.
This microservices context, or bounded context, a notion from domain-driven design \cite{Evans04}, corresponds to the minimal amount of information that the service needs to `know' in order to be able to deliver its functionality.
This lack of visibility over the context of the system and a consistent state, can make it impossible to reason about the system as a whole or to design a system with some desired high-level properties. 

Microservices arose from industry as a way for teams to deliver their software independent of other teams \cite{Zimmermann17}. 
We can trace this to Conway's law that states that an IT system starts reflecting the structure of the organization that designs the system \cite{Conway68}.
Following this argument, it is not surprising that the small functional teams that govern their development with agile methodologies and that steer clear from any complex upfront design end up using the microservices paradigm to package their deliverables.
Microservices architecture is primarily used to enable independent service deployments and evolution.
The duality of the organizational context and the information systems integrated in this context is a known challenge \cite{Nuseibeh01}.

Even though some express the opinion that the service-oriented computing and the microservices paradigm are too close to be discerned as separate disciplines (cf. \cite{Zimmermann17}), the two still represent different concepts.
Inline with this, we define a \emph{microservice} to be the smallest IT service that is invoked in different components of an application, and a \emph{service} to be a means to deliver value to a service adopter.
A service, as defined by ITIL is ``a means of delivering value to customers by facilitating outcomes customers want to achieve without the ownership of specific costs and risks'' \cite{ITIL2011}. biz and technical at the same time and business agility\footnote{ITIL 2019 introduces a new definition which we will not use.}.
Based on this definition, the service value is closely related to the displacement of costs and risks from the customer to the service provider. 




==> appendices/Standards.tex <==
\subsection{Standards}
There are three main sources of standards for privacy and privacy by design: (1) International Standardization Organization (ISO), (2) Organization for the Advancement of Structured Information Standards (OASIS), and (3) National Institute of Standards and Technologies (NIST). In this section, we discuss the advancements that the standardization bodies have made and argue that in the most part existing standards and on-going standardization efforts neither resolve nor even touch upon the topics of the disconnect between software engineering, as in service-oriented and agile development trends, and privacy engineering practices. One additional observation is that standards are not representative of the entire privacy community as the researchers who specialize in privacy engineering are usually not a part of the standardization process. We also conclude that standards are coming as an upfront prescription of how privacy engineering should be done before there is a consensus within the research and industry communities on what privacy engineering is and how it should be conducted.


The ISO/IEC 29101:2018 \cite{ISO29101} standard defines a privacy architecture framework that specifies concerns regarding PII processed by an ICT systems, lists and connects components for the implementation of such systems. The framework is intended to be a technical reference for developers of ICT systems that process PII. The architecture consists of actors, components, and concerns, as well as interactions between components. The component view (technical architecture) is presented in three layers: privacy settings, identity management and access management, and PII. The views and layers are connected to the privacy principles of ISO/IEC 29100:2011 \cite{ISO29100}. The architecture is a concise representation of a lot of enterprise process interactions w.r.t. defining how to handle data. The roles of the stakeholders (principal,  controller, handler) as well the views that defines actors, systems, and interactions between these, are a stepping stone for an architecture of a privacy solution. However, the language of the standard remains legal and organizational, even though it is intended for developers to organize and develop systems that handle PII. The mapping to PETs is recommended but not specified in enough details, the PII layer mentions some technologies but has no reference list. The relationship between the layers of the components is represented visually with block/layered diagrams, and the only other relationship is the transitive one between the privacy principles and the layers. However, these two are insufficient to draw a conclusion which PET to use when and how to design the ICT system in the first place. There is no mention of the type of system (monolith or service-oriented) or the software development cycle. The standard relies heavily on the previous iteration of the 29100:2011 to define the requirements, the privacy process, etc. Also, the responsibilities to the developers are highly unrealistic - obtaining consent from PII principals is not only an engineering decision, neither is eliciting requirements, nor is communicating the purpose of PII collection, all of which are defined as concerns that developers should take care of.

Currently under development, the ISO/IEC TR 27550 \cite{ISO27550} is a draft for a standard on privacy engineering for system life cycle processes. The integration of privacy into the engineering of systems starts with introducing privacy concerns into the life cycle processes. The core is the integration of privacy into the concepts from ISO/IEC/IEEE 15288:2015 on system life cycle processes. The processes include: acquisition, supply, human resource management, knowledge management, risk management, stakeholder needs and requirements, system requirements definition, architecture, design. The processes excludes any system and software development activities after the design of the system; so what is left out of the life cycle is any development, testing, integration, maintenance, etc. This division of design and architecture and system building is a characteristic of a waterfall-style development and much less likely to occur in current software development practices. In an annex to the main document, there is a proposition how to integrate privacy into agile software development practices and the difference between a waterfall and agile development (agile is seen as iterative waterfall): privacy concerns are added to the system under development (which is to say that the backlog includes development plans for privacy). No explanation is given on what those development plans for privacy are. There is also a dedicated role in the Sprint process called product privacy owner, who might be an external or internal member of the team and who is responsible for privacy within the organization (not within the project).

NISTIR 8062 is a document that introduces the concepts of privacy engineering and risk management for federal systems \cite{NISTIR8062}.The goals are to establish a common vocabulary through which to promote understanding and communication of privacy risk and effective implementation of privacy principles. The document is mostly a road map that provides definitions (privacy engineering, privacy as an attribute of trustworthy systems, privacy objectives), an argument how privacy engineering could benefit from systems engineering, and some should-have's for the future (e.g., ``System designers and engineers, working with policy teams, can use the objectives to help bridge the gap between high-level privacy principles and their implementation within systems.'') The privacy objectives (predictability, manageability, disassociability) are a hypothetical step towards making privacy principles actionable, as the objectives are defined as measurable outcomes to provide system engineers with clarity what privacy engineering dictates what behavior the system should exhibit. The objectives are mapped to FIPPs (Fair Information Practice Principles) to show the decomposition of high-level principles to system properties. Yet, these objectives are highly dependent on the context of the system and no guidance is provided for system engineers on how to conduct the analysis (besides a risk analysis) that would potentially yield requirements that satisfy these objectives. The choice of these three objectives as opposed to any other property and any other number of objectives, is not justified. The document provides a privacy risk model that defines some additional vocabulary, e.g., problematic data action, privacy risk factors, privacy risk characteristics, and most interestingly (for the sake of our paper) context: ``Context—the circumstances surrounding the system's processing of PII—is the foundation for the interpretative analysis necessary to understanding when a privacy boundary line has been crossed.'' This means there is an understanding of the fluidity of the context of use of ICT systems, and for that, the privacy engineering measures would be specific for each case, however, NISTIR 8062 says little about how system engineers should independently of privacy experts think about privacy, analyze, design, develop and evaluate their systems w.r.t. the changing context of use.

The PRIPARE methodology is a reference guide whose purpose it is to integrate existing privacy engineering practices and contribute a consistent body of knowledge that is easy-to-use by software engineers \cite{NotarioCMAMAKKW15}. The methodology is built on top of the traditional waterfall software development process but uses an iterative version for the phases. The different software development phases are linked with comprehensive activities and best practices for privacy engineering. The handbook connects the relevant laws and the engineering activities more closely than other methodologies. One of the missing points is the iterative development process (even though it is mentioned that the software architecture would be designed iteratively, no details are given); the methodology claims to be applicable in the case of change in the requirements for the system.

==> appendices/__latexindent_temp.tex <==
\subsection{Standards}
There are three main sources of standards for privacy and privacy by design: (1) International Standardization Organization (ISO), (2) Organization for the Advancement of Structured Information Standards (OASIS), and (3) National Institute of Standards and Technologies (NIST). In this section, we discuss the advancements that the standardization bodies have made and argue that in the most part existing standards and on-going standardization efforts neither resolve nor even touch upon the topics of the disconnect between software engineering, as in service-oriented and agile development trends, and privacy engineering practices. One additional observation is that standards are not representative of the entire privacy community as the researchers who specialize in privacy engineering are usually not a part of the standardization process. We also conclude that standards are coming as an upfront prescription of how privacy engineering should be done before there is a consensus within the research and industry communities on what privacy engineering is and how it should be conducted.


The ISO/IEC 29101:2018 \cite{ISO29101} standard defines a privacy architecture framework that specifies concerns regarding PII processed by an ICT systems, lists and connects components for the implementation of such systems. The framework is intended to be a technical reference for developers of ICT systems that process PII. The architecture consists of actors, components, and concerns, as well as interactions between components. The component view (technical architecture) is presented in three layers: privacy settings, identity management and access management, and PII. The views and layers are connected to the privacy principles of ISO/IEC 29100:2011 \cite{ISO29100}. The architecture is a concise representation of a lot of enterprise process interactions w.r.t. defining how to handle data. The roles of the stakeholders (principal,  controller, handler) as well the views that defines actors, systems, and interactions between these, are a stepping stone for an architecture of a privacy solution. However, the language of the standard remains legal and organizational, even though it is intended for developers to organize and develop systems that handle PII. The mapping to PETs is recommended but not specified in enough details, the PII layer mentions some technologies but has no reference list. The relationship between the layers of the components is represented visually with block/layered diagrams, and the only other relationship is the transitive one between the privacy principles and the layers. However, these two are insufficient to draw a conclusion which PET to use when and how to design the ICT system in the first place. There is no mention of the type of system (monolith or service-oriented) or the software development cycle. The standard relies heavily on the previous iteration of the 29100:2011 to define the requirements, the privacy process, etc. Also, the responsibilities to the developers are highly unrealistic - obtaining consent from PII principals is not only an engineering decision, neither is eliciting requirements, nor is communicating the purpose of PII collection, all of which are defined as concerns that developers should take care of.

Currently under development, the ISO/IEC TR 27550 \cite{ISO27550} is a draft for a standard on privacy engineering for system life cycle processes. The integration of privacy into the engineering of systems starts with introducing privacy concerns into the life cycle processes. The core is the integration of privacy into the concepts from ISO/IEC/IEEE 15288:2015 on system life cycle processes. The processes include: acquisition, supply, human resource management, knowledge management, risk management, stakeholder needs and requirements, system requirements definition, architecture, design. The processes excludes any system and software development activities after the design of the system; so what is left out of the life cycle is any development, testing, integration, maintenance, etc. This division of design and architecture and system building is a characteristic of a waterfall-style development and much less likely to occur in current software development practices. In an annex to the main document, there is a proposition how to integrate privacy into agile software development practices and the difference between a waterfall and agile development (agile is seen as iterative waterfall): privacy concerns are added to the system under development (which is to say that the backlog includes development plans for privacy). No explanation is given on what those development plans for privacy are. There is also a dedicated role in the Sprint process called product privacy owner, who might be an external or internal member of the team and who is responsible for privacy within the organization (not within the project).

NISTIR 8062 is a document that introduces the concepts of privacy engineering and risk management for federal systems \cite{NISTIR8062}.The goals are to establish a common vocabulary through which to promote understanding and communication of privacy risk and effective implementation of privacy principles. The document is mostly a road map that provides definitions (privacy engineering, privacy as an attribute of trustworthy systems, privacy objectives), an argument how privacy engineering could benefit from systems engineering, and some should-have's for the future (e.g., ``System designers and engineers, working with policy teams, can use the objectives to help bridge the gap between high-level privacy principles and their implementation within systems.'') The privacy objectives (predictability, manageability, disassociability) are a hypothetical step towards making privacy principles actionable, as the objectives are defined as measurable outcomes to provide system engineers with clarity what privacy engineering dictates what behavior the system should exhibit. The objectives are mapped to FIPPs (Fair Information Practice Principles) to show the decomposition of high-level principles to system properties. Yet, these objectives are highly dependent on the context of the system and no guidance is provided for system engineers on how to conduct the analysis (besides a risk analysis) that would potentially yield requirements that satisfy these objectives. The choice of these three objectives as opposed to any other property and any other number of objectives, is not justified. The document provides a privacy risk model that defines some additional vocabulary, e.g., problematic data action, privacy risk factors, privacy risk characteristics, and most interestingly (for the sake of our paper) context: ``Context—the circumstances surrounding the system's processing of PII—is the foundation for the interpretative analysis necessary to understanding when a privacy boundary line has been crossed.'' This means there is an understanding of the fluidity of the context of use of ICT systems, and for that, the privacy engineering measures would be specific for each case, however, NISTIR 8062 says little about how system engineers should independently of privacy experts think about privacy, analyze, design, develop and evaluate their systems w.r.t. the changing context of use.

The PRIPARE methodology is a reference guide whose purpose it is to integrate existing privacy engineering practices and contribute a consistent body of knowledge that is easy-to-use by software engineers \cite{NotarioCMAMAKKW15}. The methodology is built on top of the traditional waterfall software development process but uses an iterative version for the phases. The different software development phases are linked with comprehensive activities and best practices for privacy engineering. The handbook connects the relevant laws and the engineering activities more closely than other methodologies. One of the missing points is the iterative development process (even though it is mentioned that the software architecture would be designed iteratively, no details are given); the methodology claims to be applicable in the case of change in the requirements for the system.

==> include/Gaps.tex <==

%!TEX root = ../Agile_PbD.tex


We argue that privacy engineering efforts, whether they focus on methodologies as in EPbD, or they are oriented to practice, as in technologies and systems proposed by academics in security and privacy venues do not consider three aspects which are key to their integration in the software developing cycle. Concretely, we identify three problems that are often neglected in the literature leading to a disconnect that hinders the full adoption of privacy engineering based on the use of PETs at a large scale, which we describe below.

\textbf{The decontextualization of the environment in which PETs are deployed}: privacy engineering often assumes that the designer of a system has absolute control on each and every element that will be used on a system. Thus, the designer can choose the best privacy configuration for each of these elements optimizing the overall design. However, as described in Section~\ref{sec:saas}, this is far from true in current software developing practices. Designers often rely on (micro)services offered by others to build their system in an efficient manner. These microservices, in turn, are designed to operate in a variety of situations independently of their context and this has severe implications for privacy engineering. 

We note that a microservice context can be understood at many degrees of abstraction. For instance, abstraction from other processes running in the CPU, from other modules running in the server, from the functional requirements or from non-functional requirements of the application using the microservice. Microservices developers aim to create microservices that operate agnostic to the different environments in which they may be deployed.\Sf{I changed this sentence around, since making something agnostic to context is more an aspiration than a reality! Changing the order also made it less difficult to read, I hope} Typically, they assume that the application designer selects appropriate microservices that fit the development environment of the application. While this approach can be very beneficial in terms of interactions with other processes, modules, and maintaining functionality\Sf{unclear what the benefit is}; it can severely limit the privacy properties that a system embedding such microservice can provide. Effectively, the decontextualization from the environment constrains the privacy engineering capabilities of the application designer who has no means of modifying the microservice to achieve end-to-end privacy protection. We note that this effect is not particular to software engineering but has already been identified as a limitation imposed by the characteristics of components in lower layers of the supply chain [cite ICRI paper].

\Cf{does this limitation extend to PETs that are microservices (libraries or components, e.g., a privacy-preserving database), or is it the opposite: because they are super aware of the context and constraint where they can be applied, they are not dynamic. Point 3}.

\Sf{i wonder if we should use concepts like modularity and agility? (micro)services allow and encourage modularity in production of services. This brings a lot of coordination and communication overhead. Importantly, it assumes that (micro)services can be deployed independent of context. This context independence is relevant for privacy engineering, which requires some context which is a reference for all following activities that derive from data minimization. Some consequences are???: (a) the idea of context independent privacy is crazy? (b) context independent privacy means that when privacy preserving services are composed they may no longer be privacy preserving, which means we need ways to detect or evaluate this, (c) all in all it means lack of dynamism. We might need to introduce types of PETs with examples to make things more clear. We talked last time about pets as monolithic systems, pets as building blocks, and of course the matrushka doll situation that what looks like a service that integrates microservices from one level of abstraction, may itself be regarded as a microservice from another level of abstraction, e.g., tor. Would it help to systematically think through these different types of PETs for this section?}

In the reminder of this paper, when focus on privacy constraints when referring to environment decontextualization. We acknowledge that such constraints may affect or involve other constraints on functionality, or execution environment. For the sake of simplicity we conflate all of them under the umbrella of privacy.

\Sf{I think I know what you are saying here, but it would be good to discuss.}
\St{looking at our notes, we also made a difference between infrastructure service and customer/user facing service. Is that relevant here? In other words, does modularity impact pets even when applied to infrastructure services?}


\textbf{The lack of integration and composition guidelines}: At a theoretical level we do not know how the hell to compose PETs. As a result, at a practical level, because microservices privacy properties are designed independently from each other (see above), we do not know how to compose or how to integrate with PETs.   


\textbf{The tendency to neglect dynamic environments}: Monolithic, zero evolution at any abstraction level (library, component, system) regarding privacy properties nor functionality.




==> include/PETs_example.tex <==
%!TEX root = ../Agile_PbD.tex

\subsubsection{Use case: privacy-preserving billing}
\label{sec:pets_example}

Recall the billing system introduced in Section~\ref{sec:example}, but
now let us assume that the developers have implemented a privacy-preserving
\texttt{compute} service based on homomorphic commitments~\cite{BalaschRTPVG10,RialD11}
in the waterfall version. When instead of centralized the system moves
to and agile service-oriented implementation, the following challenges arise:

\noindent\emph{Challenge 1.} In agile design it is common that the system's specification changes once the system is deployed. For instance, 
assume that the customer buying the system requests a change in functionality: add a new feature to the bill computation (e.g., a time slot, 
a per-client premium, or new data collection). To implement these changes, one must change the information encrypted homomorphically, as well 
as any zero-knowledge proof used to prove that encryption is correct. These changes, however, are far from trivial and may require a new
design from scratch.

\noindent\emph{Challenge 2.} Besides changes in the specification, the use of services may change the environment in which 
PETs are deployed. Assume that the system now adds a new service \texttt{discount} that takes as input
a user's consumption to decide whether she has a discount. Even if this new service would operate on encrypted data,
the introduction of such service introduces a new data flow (discount or not discount) which, combined with the final bill value 
may leak information about the individual consumptions. Therefore, one may need to change the \texttt{compute} service 
to compensate for that leakage. 

\noindent\emph{Challenge 3.} Now consider the development team behind the \texttt{compute} service. 
While they are designing an implementing, they cannot be sure about i) which will be the requirements
of the system (Challenge 1) and under which environment, i.e., with what other services and under what configuration,
will the module be deployed. Therefore, they cannot predict what other flows there will be under deployment
and implement the adequate safeguards to ensure that the privacy guarantees provided by the privacy-preserving
computation are preserved regardless of the environment.

\noindent\emph{Challenge 4.} As a consequence, it is the designer of the overall system the one that has
to make sure that when integrating services they do not reduce each others' protection. For instance, assume
that the \texttt{store} service permits retrieving records under oblivious transfer. If the oblivious transfer and 
the homomorphic billing do not share threat model, studying the composition is hard. An open question is whether
it is possible to express threat models and consequently security definitions that compose easily.

\noindent\emph{Challenge 5.} Finally, the interaction with developers' activities is also relevant
for PETs designers. It may be that, in order to support development, e.g., debugging, 
PETs need to extend their functionalities. For instance, the \texttt{compute} module
may need to run statistics on the usage patterns to ensure that the aggregation operations
leading to the final bill are correct. \Cf{Not very happy with this last example}\Bf{I don't understand what this means.}


==> include/PrivacyEngineeringDefinition.tex <==
This paper demonstrates that research on privacy technology design and privacy engineering have implicit conceptions of software engineering that do not match current reality of the practice in the wild. In particular, we show that current work are not attuned to the shift to service-oriented architectures in combination with the use of agile methods. We show that this gap is not trivial, in fact, we argue it contributes to a mismatch between most proposals for privacy technology design and methodologies for privacy engineering on one side, and engineering practice on the other. We argue that going forward, privacy engineering needs to be cognizant of, and address challenges current software engineering practices to privacy.

To demonstrate this mismatch, we first:
\begin{itemize}
	\item provide a high level description of recent shifts in software engineering which we dub the agile turn
	\item analyze potential challenges due to the agile turn
	\item demonstrate that systematically privacy researchers have neglected or only indirectly addressed:
		\begin{enumerate}
			\item generalization and systematization of engineering aspects
			\item challenges due to service-oriented architectures
			\item challenges due to various agile methodologies that have mostly replaced waterfall approaches to software engineering
		\end{enumerate} 
\end{itemize}

To make the latter point, we look at:
\begin{enumerate}
	\item research papers that propose novel privacy designs
	\item research papers that propose privacy engineering methodologies
	\item standardization efforts that make use of these papers
\end{enumerate}

In doing so, the paper demonstrates through systematization an important gap.

\paragraph{Punting problem:}
One of the main intuitions for this paper is that software engineering is often seen secondary to computer science, or we assume that computer science abstracts away from the material conditions that surround making systems. This paper shows that such an abstraction may sometimes be useful, but at times may lead researchers to miss important problems.

Specifically, we show that systematically, privacy researchers have treated development activities and current day software architectures either as not important or as a given. In a sense, they treat software engineering as a black box. By doing so, researchers miss challenges that stem from or pertain to development activities, and the way these challenges may impact what problems are pertinent and which proposed solutions coming out of CS research are feasible. This is particularly problematic, since it casts challenges that arise out of development practices as those that also should be solved by engineers and developers. However, this neglects that if all the structures around engineering activities, and the available know-how, do not address these challenges, neither can engineers and developers. This black box approach not only misses challenges particular to different development approaches, but also exacerbates the punting problem, where legal departments think privacy is a design problem, and technical departments think the opposite, and both sides punt hoping the problem doesn't come back\footnote{Punting in American football refers to kicking the ball as far as possible to the other team, hoping that they will not come back (very quickly).} 

The treatment of software engineering as a black box is especially remarkable in proposals for privacy engineering methodologies. We find this to consistently be the case across research papers and standards proposals. We show later that abstracting away architectures and development methodologies align privacy engineering with management rather than the developers, once again not addressing the ability of design or engineer solutions.


\subsection{In focus: Privacy Engineering Research}
With research on privacy technology design, or the engineering thereof, we focus on works that develop designs of desired functionalities in a privacy preserving manner. This is work that engages in architecture, protocol or component design. With privacy engineering, we refer to research on methods, techniques and tools that aid in engineering privacy. 

While there is more to privacy research, some of it is out of our current scope. Different lines of inquiry on privacy technologies and engineering interact with research on the usability of privacy functionality, anywhere from the accessibility of privacy policies to expressiveness of privacy settings, but are distinct from such works. Similarly, the research that we cover intersects with but is not focused on technical implementations or organizational management of data protection requirements, like formalizing privacy policies and ensuring purpose based access control. This is not to say that ensuring usability and manageability of privacy is secondary or independent of privacy design and engineering, but that they are complimentary aspects, usability and manageability being out of the scope of this paper. There is also recent developments in usable security and privacy for developers. Unlike most work on PETs, this work is very cognizant of current day software engineering practices. Nevertheless, this line of research functions on another level of abstraction, focusing on how developers can use privacy preserving functionality, or how teams can be organized to manage implementation and deployment of security and privacy functionality. While this is relevant, development team issues are outside of our scope.

\sedaside{We decided to put into related work a section on what this paper is not about. Some of this content may be moved there.}

Data protection, and in particular GDPR covers more than privacy design and engineering. GDPR requires data controllers and processors to build a vision on how they can be transparent and accountable with respect to lawful collection and processing of personal data. To do so, GDPR requires these actors to be diligent with data and support their data protection vision also in design. Privacy design and engineering provides mechanisms for taking realizing such aspects in technical artifacrs.

Research in privacy design and engineering have developed independent of privacy laws like data protection, however, they intersect at different points. In addition to translating privacy frameworks into technical implementations, like data protection, privacy design and engineering provide insights, novel proposals and engineering practices that intersect with these frameworks. In particular, this intersection becomes clear, first, in the attention they pay to sensitive and/or personal information flows specific and proportionate to a purpose and, secondly, in the concept of data minimization. Using the language of contextual integrity by Helen Nissenbaum, we conceive privacy design and engineering to be the practice that proposes and implements designs that ensure privacy frameworks, like data protection and contextual integrity, informed by engineering norms, practices and technical breakthroughs. 

From this perspective, privacy design and engineering research can be seen as fundamental to achieving data protection requirements. Especially existing research on privacy enhancing designs (PETs) demonstrates novel ways to organize and design systems in a way that fulfills the given purpose and proportionality requirements, and makes it difficult to repurpose data. When taken to its full potential, it may even provide ways to fulfill functionality without collecting personal information or only collecting information that cannot be linked to individuals, making it possible for organizations to minimize the burden of complying with data protection laws. 

And, it is also in this ability to processing data without exposing it to processing parties that their differences also become evident: while from an engineering perspective, a design that leverages computation without necessarily collecting data is seen as "privacy preserving" it is not yet clear if such designs do or should mean an exit from data protection, since they may still carry risks and enhance the informational power of the organizations using such designs.

\seda{hey everyone, from here on i notice that talking about privacy design and engineering in one go is not always working (making us loose nuances). I will revisit this text and see if i should split them.}
However, privacy design and engineering research is often not sufficient to fulfill all legal data protection requirements. For example, privacy designs often do not provide principles for organizing transparency of data collection and processing. However, first, they provide ways to organize software engineering activities in order to avoid randomly collecting data and only to find a convoluted story to justify what they did so for the sake of compliance. Second, they provide a logic that can inform the technical implementation of all data protection requirements, e.g., apply data minimization to data subject access rights, data portability or auditability. 


I still need to write something about point 1 and 2, and want to later integrate point 3 and 4: 
\begin{enumerate}
	\item proportional is relative to the minimum
	\item A lot of privacy frameworks stop at the conceptual level: privacy goals, contextual analysis, threats etc. These are part and parcel of privacy engineering, however, we are particularly interested in how to design the system to fulfill those goals using state of the art privacy technologies.
	\item data minimization, as something you do before, data protection, once you have the data
	\item draw something between minimum viable product, minimum viable data
	\item see punting problem
\end{enumerate}





==> include/__latexindent_temp.tex <==
%!TEX root = ../Agile_PbD.tex
\section{Discussion}
\label{sec:discussion}

Proposals for privacy design and engineering fall short on many aspects that are essential to current software engineering practices. 
In the following, we discuss the underlying gaps, and list challenges that need to be addressed to reconcile privacy and software engineering practices. We note that although these challenges have strong technical components, they are potentially impossible to address using technical means only, requiring academics, practitioners, regulators as well as the software industry to revisit current practices.

\subsection{Mind the Gaps}
\para{The Computer Science and Engineering Schism}
Computer science researchers propose designs and methodologies that often abstract away engineering aspects with the ideal of presenting results that are valid independent of the material conditions of production or engineering. Abstraction is one path to identifying designs and methodologies that are more generalizable. Moreover, researchers like to explore novel ways of doing things, rather than constraining themselves to current industry practices. For example, most PETs aspire for solutions that avoid the dominant political economy in current software industries which relies on extractive models of data collection at the cost of privacy. 

The desire to be compatible with current software engineering practices can be difficult and at times counterproductive. Fundamental research may require a different speed than the industry, simply making it difficult to keep up with changes in the software industry. Companies may keep their engineering practices and privacy challenges secret. Finally, developers and engineers may feel better equipped to figure out how to best implement proposed designs in their working environments. This makes the ideal cut off in specificity of a privacy engineering methodology an interesting matter to study.

All these justifications aside, we show that the gap between privacy engineering solutions and actual software engineering practice also exists because research proposals assume monolithic designs and waterfall methods as the mode of software production. The abstractions used in research works hold certain assumptions about how software is produced~\cite{Birnhack12}. The papers included in our study do not address challenges associated with the very nature of how software looks like and is developed. Applying solutions that are disconnected from the agile and service-oriented nature of software, leaves too wide a gap for software developers to close. Privacy engineering in the context of services, requirements and implementation evolution, changing trust models and environments, supporting developer activities, and multiple contexts of use is far from trivial and still not a solely engineering task that developers are able to perform without fundamental research in the area. These gaps raise challenges to the operationalization of the proposed designs and methods, but also open up new research questions.

\para{Silos across sub-disciplines} Some of these implicit assumptions could be surfaced through greater cooperation across sub-disciplines in computer science. In particular, researchers working on privacy designs and engineering may benefit from collaborations with researchers in software engineering.
However, currently, these communities rarely overlap and have different conceptions of privacy and the solution space. 
For example, in the software engineering field, researchers have studied engineers' perception of privacy (cf.~\cite{HadarHATBSB18,SpiekermannC09}) and requirements engineering for privacy (cf.~\cite{Ayala-RiveraP18,ShethKM14}. Others have focused on information accountability, e.g., on translating legal documents to requirements (cf.~\cite{BreauxHR14}) and the effect of regulations on systems, discovering that high-level compliance is hard to translate into technical requirements~\cite{ShahBSWC19,ShastriWC19}.
The software engineering research field holds certain implicit beliefs -- the same way privacy engineering holds waterfall and monolithic architectures -- about privacy and about how systems are engineered. Privacy in these works usually remains on the level of data protection laws and challenges to comply with the law in technical designs. Moreover, as the mode of agile and service-orientated architectures is adopted throughout software engineering field, the modus operandi is that this is the way software is engineered; hence, software engineering research holds agile and services as implicit beliefs and does not consider the implications for privacy engineering not operating under the same assumptions.
A convergence between these fields may enrich methods and help develop privacy engineering methodologies and designs fit for modern software engineering .


\para{Standards amidst many currents}
Current efforts in standardization suffer from the same limitations as academic works. For example, the stages in the life cycle are described in standards in terms of a purpose and outcomes, e.g. \textit{``Verification and validation documentation''} in the development phase, or \textit{``Quality assured systems-of-interest accepted by the acquirer''} in the production phase. Both examples implicitly assume that there is a testing activity going on. However, the description of this activity is hard to map back to practice. For instance, development verification documentation may refer to the test themselves or their results; and quality-assurance provides no guidance regarding when or how this test should be performed. In contrast, current practices perform continuous testing \emph{both} under development and production. Furthermore, ideally, standardization should come after a technology is mature enough~\cite{Waldo06}. Given the gaps between computer science and actual engineering practice, current efforts may standardize misaligned approaches, leading to a missed opportunity for an industry wide change.

\subsection{The Elephant in the Room: The Agile Turn as a Problem}

The challenges that services and agile methods poses are difficult and beg the question whether something has to change in the way we produce software in order for privacy engineering to be feasible in the first place. There is little to excuse for privacy researchers' lack of attention to software engineering practice, but any further efforts need to also consider how current software industry practices have to change.

%the genesis of services comes with the most intrusive tracking infrastructure
Most importantly, it is possible to argue that service architectures and agile development methodologies have become the source of many privacy problems. Privacy research generally, and web measurement more specifically, has typically looked at advertising as the main driver for privacy intrusive development practices~\cite{AcarFM16,EnglehardEZRNt14,Vallina16,Zuboff19}.
From our vantage point, the irruption of software in the advertisement industry, and in particular the tools to enable massive tracking can be depicted as the first successful scalable product of service architectures. 

%advertisement is an instance of the greater data centric environment
Potentially, the advertisement tracking ecosystem can be considered an example of the greater developments in software production. The capability to continuously tap on user interactions as feedback, combined with agile development methods, enable unprecedented optimization of systems~\cite{KulynychOTG20}. This feedback is key for customer and user-centric development, continuous delivery, and rapid integration of third party services. These practices are not just steps in development methodologies that can be changed, but are baked into development environments, tools and cloud service offerings. 

%and an environment where people are just broadcasting data like there is no tomorrow, which is economically preferrable
The distributed architecture underlying services, combined with data-centric development methods and environments, ends up multiplying privacy risks. In privacy literature, distributed systems are posited as a way to decentralize data, computation and therewith power asymmetries. However, in service architectures user data captured by one service is often shared with all the others. Companies small and large inherit these practices every time they plug into service ecosystems. These ecosystems are economically attractive for lean startups that want to test minimal viable products and for industry players that want to minimize risk while pivoting business models. Data-centric development practices using current service architectures means that privacy risks are abound regardless of the size of the company or the application domain. 

%privacy engineering goes against the technical and economic wins of this environment
Service ecosystems and cloud infrastructures disadvantage organizations that want to use privacy designs and methodologies. Privacy design and methodologies, by design, limit the way in which the advantages of service ecosystems can be leveraged. For example, let us assume a company is committed to applying privacy engineering, embedding PETs in their design, and pursuing a different business model. Their developer teams will have to rely on non-standard software practices. This will require software developers who are willing to work without common toolsets and methodologies. Their users may have to tolerate systems that may lack some of the ``seamless'' experiences of data-centric designs. Investors will have to be dedicated to support such efforts. Setting up such a company, or bootstrapping privacy preserving development environments may turn out to be an uphill battle.

The diametrically opposed use of the same terminology in the software industry and privacy approaches surfaces the tensions that are at play here. Ease of service \textit{composition} increases complexity in privacy \textit{composition}; the extension of \textit{trust} to all third party service providers transforms services from `single points of failure' to `many points of failure', and externalizing business \textit{risk} and \textit{costs} comes at the \textit{cost} of increased privacy \textit{risks} and engineering \textit{costs}. 

%even if it were to be implemented, it would be in the backdrop of centralized services
Finally, even if we could consolidate terminology, practices and development environments, service architectures have gone hand in hand with the centralization of data and computation in the hands of a few dominant players like Google, Microsoft, Facebook and Amazon, making privacy engineering in this setting potentially ineffective. Some of these services have deployed privacy preserving methods, e.g., differential privacy. However, having access to immense amounts of data and creating computational dependencies can yield tremendous power, \textit{even} when the data are processed by these entities in a privacy-preserving manner~\cite{Rogaway15}. The results of such processing can have implications on society and democracy that are far greater than matters of privacy, and therefore may require political and economic interventions beyond privacy engineering and associated technical solutions~\cite{KhanP19}.


%
%\begin{itemize}
%\item  refer to all the articles that this ecosystem has gone out of control
%\item  this is not just a political problem, but also a technical issue: it is hard to do privacy and security after the agile turn and there is not much there (pen testing aside)
%\item  platform governance is a double edged sword
%\item  these systems are pushing the limits of democratic structures: bigger challenge that we do not address
%\item  facebook broke democracy: if democracy had a control system, you would have had some control before democracy broke!
%\end{itemize}


\subsection{Steps forward}
It is probably not surprising that the gap between theory and practice raises many problems that seem intractable. The problems we encounter, however, also provide many possibilities both for research and change, some of which we discuss next.

\para{Structured agile}
There are already many corrections of agile practices that may provide opportunities for rethinking its activities with an eye on privacy engineering. The introduction of agile methods in organizations have not been without its problems. These include difficulties in planning and complexity as well as the cost of agile teams and use of third party services. The responses to these problems can be thought in terms of privacy design and engineering. For example:

\begin{itemize}[nosep]
\item Proposals for \emph{structured agile}: some actors have come to make proposals for more structured agile. Efforts like this may benefit from research into, for example, how much planning is needed to enable privacy engineering? 

\item Proposals for \emph{scaled agile}: Scaled agile are proposals for large companies that have existing structures that are siloed, exploring ways to introduce more coherence among functions and departments. With scaled agile, an organization coordinates between agile teams. Such coordination may help in capturing information flows, composition of privacy designs, enabling concerted privacy engineering practices, and also addressing questions around trust. These activities may also help implement an organization-wide privacy strategy.
\end{itemize}



%\subsection{Industry and academic communities -- privacy, software, systems}
%
%In industry, a software development project requires elements of privacy engineering, software engineering, systems engineering, and more. And even though there is a running half-joke that compliance in big enterprises is a department, software engineering in practice involves many stakeholders.

%In academia, the boundaries are more rigid because the three areas are specialized and evolve independently of each other with some limited cross-pollinating ideas being exchanged. 
\para{Standardization:} Standards, if done right, hold the potential to widely disseminate privacy engineering practices in the industry. 
% A hurdle towards this goal is the disconnection between the idea of the software life cycle typically embedded in standards, and the reality of software engineering practices. 
The closing of the gaps is likely possible through standards that aspire to build a common vocabulary and to find ways to integrate knowledge from researchers, practitioners and legal experts~\cite{NISTIR8062}. 
A possible limitation is that standards need to remain abstract enough to offer flexibility of implementation across industries and practices. Every organization that obtains a standards certification tailors their practices to comply with the standards requirements. Thus, no two ways of complying with a standard are the same and standards have to allow specificities in the implementation by remaining at a higher abstraction level and introducing mainly principles to be followed.
%This is why some privacy standards and laws take a sectorial or more targeted approach to avoid too much generality. \Bf{Here we can cite HIPPA, COPPA, ISO privacy for the smart grid//}

%Business and legal people can not always understand the technologies that spur out of the booming software industry, yet, they are aware that these technologies have an impact on their enterprises and society in general. We need to respect and educate each other: (1) developers, researchers, technology-inclined people should communicate the value, capabilities, and downsides of the technologies that they use and/or develop, (2) business and legal people should communicate the implications, opportunities, and risks that they hope to enhance with the use of any technologies. None of this is possible without mutual respect and understanding that these are not two side in a battle but pieces in the same puzzle. First steps: Building a common vocabulary and finding ways to explain from both perspectives (e.g., \cite{NISTIR8062}.) 

%\item GDPR talks only about data protection. It would be useful, if privacy is not reduced to data protection in the law. Regulatory mechanism would drive the privacy engineering field as the economic incentives of the market won't do much. (cite Privacy and Data Protection by Design – from policy to engineering, they mention how privacy and data protection should not be reduced to protection of data only)

\para{The limits and potentials of purpose limitation} One way to mitigate the many challenges that agile practices in service architectures pose to privacy design and methodologies is through regulation. Very much like proposals coming from privacy research, data protection laws promote minimizing collection of data and restricting its use to a specific purpose, although not necessarily technically. 

Limiting data collection to a purpose only contractually is not sufficient to curb the very broad data collection and dissemination practices that services architectures and agile development practices have normalized. 
In current software development practices, once data are collected for a given purpose, they can be fed into service architectures and used in agile processes as long as it is done transparently. To guarantee transparency, regulation promotes contractual obligations encoded in terms of service or privacy policies. In the end of the day, regulation does not encourage purpose limitation at the technical implementation and thus software developers rarely design software with this principle.
%This is a missed opportunity to use protocols with mathematical guarantees that constrain what operations can be done on the data given the purpose of its collection.  
It is promising that regulators have recently started looking at privacy intrusive infrastructural designs from a purpose limitation perspective. This is the case in a recent inquiry into Google and IAB's Real-Time Bidding standard~\cite{Ryan18}, as well as the recent complaint that Microsoft ProPlus telemetry data violates data protection and in particular purpose limitation~\cite{privacyCompany}. 
The notion of purpose limitation has the potential to appeal to agile teams that produce services because the existing metaphors in the field are closely related.
Limiting the scope of what is done and how, through concepts such as bounded context and doing one thing well, is at the heart of software engineering practices. 
Introducing purpose limitation could potentially ripple throughout the end-to-end designs and tie the legal nature of purpose limitation to the technical implementation. 
How data protection laws and software engineering methods combined can better ensure data minimization is enforced in service ecosystems is an interesting point of future inquiry.

\para{Circling back to computer science and engineering}

The challenges above may determine the future of privacy designs and privacy engineering. In the meantime some low-hanging fruits can be addressed from a technical perspective:

\begin{enumerate}[nosep]
\item Empirical and Measurement Research: Capture in depth the challenges modularity, evolution, distributed trust and novel development methods raise for privacy designs and methodologies. Conduct empirical studies of current software engineering practices with an eye on privacy engineering, experiment with ways to introduce privacy designs and engineering methods. Expand work on web measurement from the current focus on advertisement to study software infrastructures.
\item Design for agile and services: Explore PETs that can be updated, that enable new encoding, or are composable. Study different models of PET composition using and going beyond service orchestration and choreography.
\item Support Developers: Consider ways in which current software engineering practices can be done in a privacy preserving manner: e.g., privacy preserving monitoring of service environment. Introduce testing suits and evaluation methods for (composition in) PETs. Study and mitigate privacy implications of developer activities like dark launches, parallel development, continuous integration. Engage in "brownfield" privacy engineering, i.e., retrofitting privacy into legacy systems in agile service environments.
\end{enumerate}

\Bt{
    New points to bring into the discussion:
    \begin{itemize}
        \item all these aspects that we evaluate the methodologies on (criteria from Table 2), are there methodologies that deal with them without the privacy aspect, and if yes, how? Is it possible to capture all these aspects within a methodology or is it a single-case treatment that we can hope for at best?
        \item 50\% of the PETs articles are on analysis and attacks -- could be of great value to package these as tests for new systems, or evaluation suites (are we vulnerable to known problems? extract the problems from the context, organize them in taxonomies of attacks and analysis, create standardized tests for new privacy systems)
        \item service composition layer as the almighty oracle --> even though everything is partitioned, in an enterprise context, there is usually/almost always a point where everything comes together (business transactions have to be verified, we can't expect that the payment of a bill will be actually received). However, data flows are of actual problem, as generating more data flows isn't a problem in services. Business rule engines, integration test suites, transactions, we always have a way to test the end result of an operation carried out in a system. Yet, distributed systems are notorious for their consistency issues (what do we do with the CAP theorem?) 
        \item microservices and choreography are snake oil, but the service-orientation isn't. Everyone might be talking how they do microservices but at the end of the day, it's only a monolithic microservices architecture. We can't let go of all control and the illusion of flexibility might come at a greater cost that the PR it generates (some trends are practiced so that companies can attract top talent or to satisfy market dynamics, not because of a real need) As long as we go beyond the hype and acknowledge that there is still control, we might be able to (1) study where who has control over what, (2) design systems that make use of the control mechanisms
    \end{itemize}
}


%The majority of software development just does not happen from a blank slate \cite{LiWE19}

%Is one of our goals that privacy engineering supports some of the issues we identify as grand challenges in the discussion?
%Can we even do it, or do we just need to change the business models and there is nothing that can be done short of that.

%		\item data for pivoting companies, disrupting new domains. e.g., Waze patent shows that they collect income, house ownership, mortgage data about their users. You can tell they want to pivot. What do we say?











